PBCS : Efficient Exploration and Exploitation Using a Synergy between Reinforcement Learning and Motion Planning

The exploration-exploitation trade-off is at the heart of reinforcement learning (RL). However, most continuous control benchmarks used in recent RL research only require local exploration. This led to the development of algorithms that have basic exploration capabilities, and behave poorly in benchmarks that require more versatile exploration. For instance, as demonstrated in our empirical study, state-of-the-art RL algorithms such as DDPG and TD3 are unable to steer a point mass in even small 2D mazes. In this paper, we propose a new algorithm called "Plan, Backplay, Chain Skills" (PBCS) that combines motion planning and reinforcement learning to solve hard exploration environments. In a first phase, a motion planning algorithm is used to find a single good trajectory, then an RL algorithm is trained using a curriculum derived from the trajectory, by combining a variant of the Backplay algorithm and skill chaining. We show that this method outperforms state-of-the-art RL algorithms in 2D maze environments of various sizes, and is able to improve on the trajectory obtained by the motion planning phase.

==> Makefile <==
SVG = $(wildcard inkscape/*.svg)
PNG = $(wildcard images/*.{png,pdf})
DOTS = $(wildcard dots/*.tex)
MP4 = $(wildcard *.mp4)

PDFTEX = $(subst inkscape/,build/,$(SVG:.svg=.pdf))
PDFDOTS = $(subst dots/,build/,$(DOTS:.tex=.pdf))
BUILD = $(PDFTEX) $(PDFDOTS)

MP4_FRAME = $(MP4:.mp4=_frame.jpg)
#SMALL_PNG = $(PNG:.png=_small.png)

DEPS = $(PDFTEX) $(PNG) $(MP4_FRAME) ex.bib $(BUILD) results.tex results_big.tex 

all: ex.pdf ex_arxiv.pdf

.PHONY: fast
fast: ex.tex $(DEPS)
	pdflatex ex.tex

.PHONY: diff
diff:
	git show $(OLD):./ex.tex > tmp1.tex
	git show $(NEW):./ex.tex > tmp2.tex
	latexdiff tmp1.tex tmp2.tex > diff.tex
	pdflatex diff.tex
	bibtex diff.aux
	pdflatex diff.tex
	pdflatex diff.tex
	rm tmp1.tex tmp2.tex

ex.bib: zotero.bib
	perl -0777 -pe 's/note = \{[^}]*\}/note={}/g' $< > $@
	sed -i 's/journal = {\(.*\) \[.*\]}/journal = {\1}/' $@

ex.pdf: ex.tex $(DEPS) ex.bib
	-pdflatex ex.tex
	bibtex ex
	-pdflatex ex.tex
	-pdflatex ex.tex

ex_arxiv.pdf: ex.tex $(DEPS) ex.bib
	sed 's/Enabledfalse/Enabledtrue/' ex.tex > ex_arxiv.tex
	sed -i 's/bibliography{ex}/bibliography{ex_arxiv}/' ex_arxiv.tex
	cp ex.bib ex_arxiv.bib
	-pdflatex ex_arxiv.tex
	bibtex ex_arxiv
	-pdflatex ex_arxiv.tex
	-pdflatex ex_arxiv.tex
	cd .. && tar cvzf pbcs_arxiv.tar.gz 202004_icann_pbcs

build/%.pdf: inkscape/%.svg
	mkdir -p build
	#inkscape -C -z --file=$< --export-pdf=$(@:.pdf_tex=.pdf) --export-latex
	inkscape -C -z --file=$< --export-pdf=$(@:.pdf_tex=.pdf)

%_frame.jpg: %.mp4
	ffmpeg -ss 00:00:00 -i $<  -vframes 1 -q:v 2 $(@:.mp4=_frame.jpg)

build/%.pdf: dots/%.pdf
	cp $< $@

dots/%.pdf: dots/%.tex
	cd dots; lualatex --shell-escape $(notdir $<); rm -f *-fig*.tex

build/%.pdf: images/%.svg
	mkdir -p build
	inkscape $< --export-pdf $@

.PHONY: clean

clean:
	-rm -f *.pdf_tex *.pdf *.aux *.log *.out *.blg *.bbl \
		*.bcf *.nav *.run.xml *.snm *.toc *.vrb $(BUILD) *_frame.jpg \
		ex.bib diff.*


